Deep Bayesian Bandits Showdown: An Empirical Comparison of Bayesian Deep Networks for Thompson Sampling

Recent advances in deep reinforcement learning have made significant strides in performance on applications such as Go and Atari games. However, developing practical methods to balance exploration and exploitation in complex domains remains largely unsolved. Thompson Sampling and its extension to reinforcement learning provide an elegant approach to exploration that only requires access to posterior samples of the model. At the same time, advances in approximate Bayesian methods have made posterior approximation for flexible neural network models practical. Thus, it is attractive to consider approximate Bayesian neural networks in a Thompson Sampling framework. To understand the impact of using an approximate posterior on Thompson Sampling, we benchmark well-established and recently developed methods for approximate posterior sampling combined with Thompson Sampling over a series of contextual bandit problems. We found that many approaches that have been successful in the supervised learning setting underperformed in the sequential decision-making scenario. In particular, we highlight the challenge of adapting slowly converging uncertainty estimates to the online setting.

==> tables/tab_app_chrome_time.tex <==
\begin{tabular}{llllll}
 & $\delta = 0.5$ & $\delta = 0.7$ & $\delta = 0.9$ & $\delta = 0.95$ & $\delta = 0.99$ \\
\midrule
AlphaDivergence (1) & $1669.73 \pm 98.23$& $1736.91 \pm 128.92$& $1788.96 \pm 191.83$& $2271.48 \pm 169.18$& $2351.98 \pm 169.98$ \\
AlphaDivergence & $1733.73 \pm 237.92$& $2398.18 \pm 181.66$& $1733.50 \pm 174.96$& $2332.87 \pm 154.71$& $2627.66 \pm 489.16$ \\
AlphaDivergence-SL & $831.76 \pm 153.41$& $1229.94 \pm 351.34$& $1022.87 \pm 259.69$& $1100.53 \pm 251.75$& $1129.44 \pm 231.47$ \\
BBB & $671.17 \pm 49.36$& $983.12 \pm 66.11$& $737.75 \pm 46.62$& $968.72 \pm 123.41$& $1039.11 \pm 110.18$ \\
BBB-MR & $623.04 \pm 163.27$& $905.40 \pm 180.76$& $751.51 \pm 209.57$& $808.51 \pm 133.90$& $978.27 \pm 327.24$ \\
BBB-SL & $716.76 \pm 249.93$& $967.40 \pm 251.41$& $825.89 \pm 207.49$& $838.65 \pm 127.50$& $927.24 \pm 228.31$ \\
BootstrappedNN & $988.05 \pm 114.28$& $945.33 \pm 50.54$& $1014.13 \pm 76.82$& $946.70 \pm 47.61$& $980.44 \pm 78.48$ \\
BootstrappedNN-MR & $52.61 \pm 7.11$& $76.38 \pm 12.39$& $65.92 \pm 9.19$& $74.58 \pm 9.93$& $78.15 \pm 16.27$ \\
BootstrappedNN-SL & $55.66 \pm 8.64$& $82.94 \pm 12.17$& $74.69 \pm 13.07$& $79.75 \pm 9.35$& $87.68 \pm 22.21$ \\
Dropout & $139.05 \pm 12.52$& $204.83 \pm 18.66$& $135.01 \pm 8.09$& $206.56 \pm 23.76$& $203.35 \pm 23.08$ \\
Dropout-MR & $29.06 \pm 3.76$& $40.66 \pm 6.21$& $36.62 \pm 4.42$& $40.20 \pm 5.06$& $40.97 \pm 6.40$ \\
Dropout-SL & $388.03 \pm 32.41$& $574.09 \pm 78.17$& $496.63 \pm 47.78$& $531.06 \pm 50.80$& $533.64 \pm 47.09$ \\
GP & $6992.01 \pm 843.03$& $11816.10 \pm 2234.71$& $7805.21 \pm 580.05$& $9538.26 \pm 575.82$& $9678.15 \pm 509.54$ \\
NeuralLinear & $145.34 \pm 11.05$& $156.91 \pm 6.55$& $158.68 \pm 14.53$& $148.49 \pm 8.25$& $150.21 \pm 10.17$ \\
NeuralLinear-MR & $152.44 \pm 9.85$& $226.13 \pm 19.02$& $201.52 \pm 17.71$& $208.11 \pm 15.08$& $218.42 \pm 19.22$ \\
NeuralLinear-SL & $130.05 \pm 9.36$& $185.12 \pm 16.18$& $162.00 \pm 13.07$& $177.28 \pm 14.17$& $181.22 \pm 20.29$ \\
RMS & $100.00 \pm 10.84$& $100.00 \pm 4.95$& $100.00 \pm 9.88$& $100.00 \pm 5.57$& $100.00 \pm 6.64$ \\
RMS-MR & $41.91 \pm 5.83$& $62.92 \pm 12.30$& $56.52 \pm 8.86$& $59.12 \pm 6.68$& $61.63 \pm 8.31$ \\
RMS-SL & $82.39 \pm 8.65$& $125.22 \pm 13.86$& $108.02 \pm 17.78$& $116.88 \pm 12.16$& $115.61 \pm 12.01$ \\
SGFS & $159.46 \pm 17.80$& $231.76 \pm 22.03$& $159.61 \pm 9.20$& $226.00 \pm 25.11$& $235.07 \pm 29.12$ \\
SGFS-MR & $175.29 \pm 41.89$& $243.81 \pm 66.14$& $212.24 \pm 33.71$& $234.78 \pm 56.58$& $223.36 \pm 23.22$ \\
SGFS-SL & $70.57 \pm 24.01$& $104.27 \pm 20.63$& $85.44 \pm 14.36$& $93.94 \pm 14.80$& $99.58 \pm 26.61$ \\
ConstSGD & $106.69 \pm 9.69$& $111.83 \pm 6.90$& $111.12 \pm 12.28$& $111.83 \pm 5.34$& $109.24 \pm 4.78$ \\
ConstSGD-MR & $11.28 \pm 2.71$& $16.10 \pm 3.24$& $14.68 \pm 5.65$& $14.90 \pm 2.74$& $15.97 \pm 4.28$ \\
ConstSGD-SL & $43.87 \pm 7.41$& $68.37 \pm 10.66$& $57.62 \pm 9.66$& $61.75 \pm 7.87$& $70.30 \pm 17.95$ \\
EpsGreedyRMS & $96.75 \pm 9.48$& $99.18 \pm 3.34$& $98.85 \pm 10.05$& $98.15 \pm 5.16$& $99.42 \pm 6.33$ \\
EpsGreedyRMS-SL & $164.45 \pm 19.10$& $243.03 \pm 26.72$& $211.23 \pm 23.35$& $231.10 \pm 21.48$& $243.69 \pm 35.48$ \\
EpsGreedyRMS-MR & $40.68 \pm 5.82$& $57.36 \pm 6.71$& $49.52 \pm 6.89$& $53.49 \pm 5.57$& $57.92 \pm 8.77$ \\
LinDiagPost & $12.60 \pm 1.97$& $17.06 \pm 2.54$& $13.48 \pm 1.53$& $19.01 \pm 3.18$& $13.94 \pm 1.39$ \\
LinDiagPost-MR & $10.06 \pm 1.12$& $14.07 \pm 1.39$& $12.41 \pm 1.23$& $13.88 \pm 1.98$& $15.31 \pm 2.56$ \\
LinDiagPost-SL & $10.93 \pm 1.57$& $15.24 \pm 2.60$& $14.52 \pm 1.85$& $17.27 \pm 2.91$& $18.28 \pm 2.50$ \\
LinDiagPrecPost & $11.98 \pm 1.50$& $19.67 \pm 2.98$& $13.86 \pm 1.81$& $18.00 \pm 2.38$& $14.07 \pm 1.24$ \\
LinDiagPrecPost-MR & $10.13 \pm 1.21$& $14.91 \pm 2.00$& $14.08 \pm 2.07$& $15.65 \pm 1.99$& $16.71 \pm 2.50$ \\
LinDiagPrecPost-SL & $10.80 \pm 1.68$& $15.41 \pm 2.25$& $14.96 \pm 2.73$& $16.87 \pm 2.17$& $19.21 \pm 3.15$ \\
LinGreedy & $10.19 \pm 1.76$& $11.35 \pm 1.11$& $12.76 \pm 1.52$& $12.51 \pm 0.90$& $12.98 \pm 0.93$ \\
LinGreedy ($\epsilon =0.01$) & $8.99 \pm 1.63$& $9.57 \pm 0.57$& $10.82 \pm 1.37$& $11.59 \pm 1.36$& $13.94 \pm 1.21$ \\
LinGreedy ($\epsilon =0.05$) & $9.25 \pm 1.63$& $9.51 \pm 0.53$& $10.01 \pm 1.20$& $9.70 \pm 0.65$& $11.44 \pm 1.02$ \\
LinPost & $12.27 \pm 1.45$& $18.44 \pm 3.03$& $13.93 \pm 1.74$& $19.33 \pm 3.63$& $14.05 \pm 1.16$ \\
LinPost-MR & $9.61 \pm 0.54$& $13.88 \pm 1.13$& $12.38 \pm 1.50$& $13.25 \pm 0.85$& $13.47 \pm 0.60$ \\
LinPost-SL & $10.58 \pm 1.39$& $15.59 \pm 2.93$& $15.06 \pm 2.66$& $16.78 \pm 1.88$& $19.00 \pm 2.74$ \\
LinFullDiagPost & $13.77 \pm 1.72$& $15.76 \pm 2.09$& $15.34 \pm 1.90$& $14.79 \pm 2.27$& $15.90 \pm 1.57$ \\
LinFullDiagPost-MR & $11.75 \pm 1.96$& $15.86 \pm 1.70$& $14.54 \pm 1.78$& $16.15 \pm 2.15$& $17.86 \pm 1.83$ \\
LinFullDiagPost-SL & $11.49 \pm 1.26$& $17.21 \pm 3.64$& $15.72 \pm 1.84$& $16.57 \pm 1.58$& $18.31 \pm 2.67$ \\
LinFullDiagPrecPost & $13.67 \pm 1.99$& $14.37 \pm 0.83$& $15.55 \pm 1.83$& $14.97 \pm 2.53$& $15.75 \pm 1.58$ \\
LinFullDiagPrecPost-MR & $11.54 \pm 1.31$& $15.77 \pm 1.85$& $14.09 \pm 2.31$& $15.37 \pm 2.07$& $16.25 \pm 2.18$ \\
LinFullDiagPrecPost-SL & $11.65 \pm 1.36$& $15.93 \pm 1.78$& $16.05 \pm 3.09$& $17.56 \pm 2.26$& $18.35 \pm 2.06$ \\
LinFullPost & $14.27 \pm 2.23$& $19.66 \pm 2.82$& $15.56 \pm 1.74$& $19.69 \pm 3.51$& $15.89 \pm 1.40$ \\
LinFullPost-MR & $12.83 \pm 2.05$& $18.12 \pm 2.85$& $16.28 \pm 2.45$& $17.89 \pm 1.91$& $21.29 \pm 3.32$ \\
LinFullPost-SL & $12.45 \pm 1.62$& $18.42 \pm 2.10$& $18.84 \pm 3.23$& $19.77 \pm 2.60$& $20.18 \pm 2.42$ \\
ParamNoise & $175.91 \pm 14.23$& $188.08 \pm 9.14$& $191.42 \pm 22.73$& $181.11 \pm 8.01$& $187.83 \pm 11.38$ \\
ParamNoise-MR & $39.18 \pm 4.33$& $56.57 \pm 7.51$& $50.47 \pm 6.14$& $56.82 \pm 7.35$& $60.55 \pm 11.48$ \\
ParamNoise-SL & $10.67 \pm 1.39$& $15.75 \pm 2.08$& $14.26 \pm 1.67$& $15.40 \pm 2.50$& $15.40 \pm 1.70$ \\
Uniform & \bm{$0.16 \pm 0.02$}& \bm{$0.23 \pm 0.03$}& \bm{$0.21 \pm 0.03$}& \bm{$0.23 \pm 0.03$}& \bm{$0.23 \pm 0.03$} \\
\bottomrule
\end{tabular}


==> tables/tab_main_simple_regret.tex <==
\begin{tabular}{llllll}
 & Mushroom & Statlog & Covertype & Financial & Jester \\
\midrule
AlphaDivergence (1) & $51.57 \pm 0.31$& $17.48 \pm 1.51$& $30.71 \pm 1.41$& $19.45 \pm 0.80$& $68.37 \pm 0.95$ \\
AlphaDivergence & $51.20 \pm 0.32$& $13.32 \pm 1.34$& $33.71 \pm 1.72$& $26.86 \pm 1.22$& $67.35 \pm 0.91$ \\
AlphaDivergence-SL & $51.24 \pm 0.36$& $22.47 \pm 1.08$& $59.61 \pm 0.31$& $60.74 \pm 5.12$& $64.64 \pm 0.86$ \\
BBB & \bm{$0.63 \pm 0.17$}& $12.47 \pm 1.59$& $56.84 \pm 2.21$& $19.00 \pm 1.37$& $66.76 \pm 0.82$ \\
BBB-MR & $8.94 \pm 2.62$& $24.91 \pm 0.28$& $60.37 \pm 0.59$& $46.47 \pm 3.57$& $63.18 \pm 0.85$ \\
BBB-SL & $0.82 \pm 0.16$& $1.26 \pm 0.26$& $34.62 \pm 0.75$& $7.46 \pm 0.57$& $68.79 \pm 0.93$ \\
BootstrappedNN & $2.43 \pm 0.49$& $0.27 \pm 0.04$& $22.47 \pm 0.25$& $3.29 \pm 0.36$& $70.29 \pm 0.73$ \\
BootstrappedNN-MR & $1.26 \pm 0.17$& $0.67 \pm 0.10$& $29.81 \pm 0.36$& $3.37 \pm 0.32$& $59.96 \pm 0.74$ \\
BootstrappedNN-SL & $1.44 \pm 0.25$& \bm{$0.26 \pm 0.03$}& $21.38 \pm 0.35$& $6.76 \pm 0.64$& $67.17 \pm 0.68$ \\
Dropout & $2.59 \pm 1.09$& $1.34 \pm 0.55$& $28.34 \pm 0.42$& $11.42 \pm 0.70$& $63.47 \pm 0.80$ \\
Dropout-MR & \bm{$0.68 \pm 0.14$}& $0.67 \pm 0.13$& $27.96 \pm 0.36$& $6.04 \pm 0.47$& $61.04 \pm 0.74$ \\
Dropout-SL & $2.37 \pm 1.07$& $1.38 \pm 0.44$& $23.28 \pm 0.40$& $8.70 \pm 0.87$& $63.65 \pm 0.78$ \\
GP & $10.66 \pm 0.85$& $3.80 \pm 0.74$& $45.65 \pm 0.89$& \bm{$0.22 \pm 0.07$}& $74.38 \pm 1.18$ \\
NeuralLinear & \bm{$0.46 \pm 0.12$}& $0.32 \pm 0.04$& $25.30 \pm 0.33$& $2.74 \pm 0.08$& $70.67 \pm 0.66$ \\
NeuralLinear-MR & $1.10 \pm 0.16$& $0.56 \pm 0.05$& $25.30 \pm 0.36$& $3.98 \pm 0.09$& $67.80 \pm 0.69$ \\
NeuralLinear-SL & $0.84 \pm 0.12$& \bm{$0.20 \pm 0.03$}& $23.89 \pm 0.37$& $5.04 \pm 0.64$& $67.80 \pm 0.65$ \\
RMS & $5.02 \pm 1.47$& $2.14 \pm 0.75$& $23.71 \pm 0.34$& $7.36 \pm 0.69$& $65.68 \pm 0.77$ \\
RMS-MR & $2.82 \pm 1.07$& $1.72 \pm 0.38$& $28.73 \pm 0.47$& $5.73 \pm 0.53$& $64.53 \pm 0.88$ \\
RMS-SL & $1.22 \pm 0.16$& $0.56 \pm 0.21$& $23.00 \pm 0.35$& $8.29 \pm 0.61$& $68.15 \pm 0.69$ \\
SGFS & $4.11 \pm 0.83$& $2.41 \pm 0.45$& $33.57 \pm 0.86$& $16.76 \pm 0.53$& $64.75 \pm 0.85$ \\
SGFS-MR & $2.47 \pm 0.47$& $1.05 \pm 0.14$& $28.73 \pm 0.32$& $6.74 \pm 0.64$& $62.03 \pm 0.74$ \\
SGFS-SL & $0.87 \pm 0.13$& $0.87 \pm 0.09$& $33.62 \pm 0.42$& $19.12 \pm 0.88$& $72.20 \pm 1.64$ \\
ConstSGD & $19.57 \pm 3.39$& $5.94 \pm 1.46$& \bm{$15.63 \pm 0.95$}& $86.75 \pm 3.92$& $68.48 \pm 0.95$ \\
ConstSGD-MR & $0.85 \pm 0.17$& $6.34 \pm 1.10$& $17.25 \pm 0.57$& $40.63 \pm 2.73$& $67.64 \pm 0.73$ \\
ConstSGD-SL & $37.01 \pm 4.26$& $2.22 \pm 0.78$& \bm{$16.15 \pm 0.30$}& $42.59 \pm 4.82$& $69.47 \pm 0.97$ \\
EpsGreedyRMS & $2.63 \pm 1.09$& $0.55 \pm 0.17$& $23.58 \pm 0.34$& $5.83 \pm 0.43$& $65.53 \pm 0.89$ \\
EpsGreedyRMS-SL & $1.59 \pm 0.21$& $0.62 \pm 0.24$& $23.93 \pm 0.32$& $3.32 \pm 0.37$& $65.53 \pm 0.76$ \\
EpsGreedyRMS-MR & $1.30 \pm 0.19$& $1.26 \pm 0.46$& $27.21 \pm 0.43$& $3.73 \pm 0.43$& $62.04 \pm 0.66$ \\
LinDiagPost & $16.67 \pm 0.40$& $37.05 \pm 0.36$& $95.17 \pm 0.22$& $2.08 \pm 0.05$& \bm{$53.75 \pm 0.51$} \\
LinDiagPost-MR & $6.85 \pm 2.19$& $29.96 \pm 0.30$& $61.52 \pm 0.37$& $10.95 \pm 0.18$& $55.44 \pm 0.62$ \\
LinDiagPost-SL & $13.93 \pm 2.06$& $13.97 \pm 0.21$& $41.70 \pm 0.31$& \bm{$0.16 \pm 0.02$}& $56.03 \pm 0.79$ \\
LinDiagPrecPost & $8.56 \pm 1.53$& $6.44 \pm 0.18$& $32.97 \pm 0.31$& $1.04 \pm 0.04$& \bm{$54.31 \pm 0.71$} \\
LinDiagPrecPost-MR & $15.55 \pm 3.12$& $5.83 \pm 0.15$& $33.40 \pm 0.33$& $3.21 \pm 0.08$& $54.92 \pm 0.64$ \\
LinDiagPrecPost-SL & $12.16 \pm 1.73$& $6.62 \pm 0.16$& $33.17 \pm 0.35$& \bm{$0.12 \pm 0.04$}& \bm{$54.35 \pm 0.62$} \\
LinGreedy & $13.62 \pm 2.04$& $9.35 \pm 0.76$& $34.75 \pm 0.33$& $0.50 \pm 0.15$& $55.32 \pm 0.82$ \\
LinGreedy ($\epsilon =0.01$) & $1.74 \pm 0.22$& $8.31 \pm 0.27$& $33.73 \pm 0.32$& $0.97 \pm 0.10$& $55.87 \pm 0.77$ \\
LinGreedy ($\epsilon =0.05$) & $4.67 \pm 0.35$& $11.54 \pm 0.26$& $36.61 \pm 0.34$& $5.12 \pm 0.23$& $57.37 \pm 0.60$ \\
LinPost & $5.31 \pm 0.68$& $6.47 \pm 0.15$& $33.02 \pm 0.34$& $1.17 \pm 0.04$& \bm{$54.91 \pm 0.66$} \\
LinPost-MR & $6.67 \pm 1.95$& $7.57 \pm 0.19$& $34.25 \pm 0.33$& $6.89 \pm 0.11$& $55.27 \pm 0.66$ \\
LinPost-SL & $13.69 \pm 1.73$& $6.46 \pm 0.17$& $32.50 \pm 0.32$& $0.24 \pm 0.03$& $56.15 \pm 0.77$ \\
LinFullDiagPost & $83.94 \pm 1.32$& $20.92 \pm 0.28$& $73.04 \pm 0.33$& $0.32 \pm 0.03$& $57.29 \pm 0.73$ \\
LinFullDiagPost-MR & $0.85 \pm 0.13$& $12.24 \pm 0.20$& $36.09 \pm 0.37$& $2.70 \pm 0.07$& $57.81 \pm 0.65$ \\
LinFullDiagPost-SL & $0.69 \pm 0.10$& $11.38 \pm 0.22$& $36.42 \pm 0.38$& $5.65 \pm 0.37$& $57.18 \pm 0.66$ \\
LinFullDiagPrecPost & $2.85 \pm 0.37$& $6.44 \pm 0.18$& $33.01 \pm 0.31$& \bm{$0.18 \pm 0.03$}& $56.63 \pm 0.69$ \\
LinFullDiagPrecPost-MR & $2.25 \pm 0.34$& $6.21 \pm 0.16$& $32.84 \pm 0.32$& $0.56 \pm 0.04$& $55.90 \pm 0.67$ \\
LinFullDiagPrecPost-SL & $2.05 \pm 0.16$& $6.14 \pm 0.17$& $32.77 \pm 0.33$& $1.15 \pm 0.10$& $55.54 \pm 0.77$ \\
LinFullPost & $1.75 \pm 0.29$& $6.12 \pm 0.15$& $33.16 \pm 0.32$& $0.19 \pm 0.03$& $57.43 \pm 0.71$ \\
LinFullPost-MR & $1.27 \pm 0.16$& $6.00 \pm 0.18$& $33.01 \pm 0.33$& $1.44 \pm 0.04$& $55.72 \pm 0.67$ \\
LinFullPost-SL & $2.11 \pm 0.31$& $6.21 \pm 0.18$& $32.99 \pm 0.34$& $1.25 \pm 0.06$& $55.94 \pm 0.57$ \\
ParamNoise & $1.36 \pm 0.20$& $0.66 \pm 0.13$& $21.82 \pm 0.30$& $15.32 \pm 0.82$& $64.94 \pm 0.75$ \\
ParamNoise-MR & $1.08 \pm 0.17$& $0.83 \pm 0.17$& $24.32 \pm 0.37$& $15.45 \pm 0.34$& $66.91 \pm 0.83$ \\
ParamNoise-SL & \bm{$0.74 \pm 0.17$}& $0.62 \pm 0.20$& $23.06 \pm 0.35$& $4.98 \pm 0.69$& $63.22 \pm 0.64$ \\
Uniform & $100.00 \pm 1.66$& $100.00 \pm 0.27$& $100.00 \pm 0.20$& $100.00 \pm 1.58$& $100.00 \pm 1.22$ \\
\bottomrule
\end{tabular}


==> tables/tab_main_time.tex <==
\begin{tabular}{llllll}
 & Mushroom & Statlog & Covertype & Financial & Jester \\
\midrule
AlphaDivergence (1) & $560.20 \pm 46.72$& $735.02 \pm 55.50$& $258.25 \pm 14.97$& $10289.67 \pm 827.51$& $1663.50 \pm 143.87$ \\
AlphaDivergence & $547.82 \pm 36.53$& $746.48 \pm 57.83$& $258.34 \pm 14.62$& $10407.11 \pm 858.31$& $1662.82 \pm 145.74$ \\
AlphaDivergence-SL & $498.78 \pm 120.20$& $568.54 \pm 61.40$& $300.86 \pm 57.50$& $5517.58 \pm 1612.75$& $1033.02 \pm 215.51$ \\
BBB & $264.64 \pm 11.42$& $327.16 \pm 19.62$& $146.61 \pm 10.23$& $4569.10 \pm 278.55$& $799.22 \pm 71.61$ \\
BBB-MR & $227.28 \pm 46.01$& $288.37 \pm 55.36$& $61.35 \pm 12.44$& $5537.82 \pm 1035.35$& $814.01 \pm 117.19$ \\
BBB-SL & $247.48 \pm 33.11$& $315.44 \pm 55.78$& $78.16 \pm 12.39$& $6282.18 \pm 1787.78$& $926.67 \pm 269.69$ \\
BootstrappedNN & $1032.55 \pm 61.06$& $1033.71 \pm 63.65$& $1061.96 \pm 85.07$& $973.91 \pm 77.44$& $974.03 \pm 75.80$ \\
BootstrappedNN-MR & $91.13 \pm 9.23$& $67.81 \pm 9.11$& $79.04 \pm 16.50$& $61.76 \pm 9.45$& $66.32 \pm 10.25$ \\
BootstrappedNN-SL & $109.20 \pm 20.02$& $68.67 \pm 7.26$& $82.75 \pm 10.40$& $77.57 \pm 23.63$& $75.14 \pm 12.67$ \\
Dropout & $145.85 \pm 7.07$& $149.43 \pm 10.07$& $172.68 \pm 12.85$& $132.70 \pm 10.60$& $131.35 \pm 6.79$ \\
Dropout-MR & $50.02 \pm 4.34$& $35.26 \pm 2.99$& $40.45 \pm 3.15$& $37.52 \pm 5.32$& $36.90 \pm 5.58$ \\
Dropout-SL & $399.08 \pm 30.09$& $467.46 \pm 42.40$& $328.78 \pm 26.29$& $562.34 \pm 79.47$& $484.15 \pm 57.88$ \\
GP & $4400.76 \pm 388.68$& $5764.29 \pm 365.29$& $1789.18 \pm 267.01$& $8223.17 \pm 589.89$& $7353.49 \pm 487.87$ \\
NeuralLinear & $137.23 \pm 5.64$& $207.10 \pm 14.55$& $213.15 \pm 14.33$& $212.58 \pm 15.98$& $197.54 \pm 17.03$ \\
NeuralLinear-MR & $177.61 \pm 12.09$& $266.55 \pm 15.62$& $208.71 \pm 16.18$& $277.01 \pm 23.85$& $234.43 \pm 18.30$ \\
NeuralLinear-SL & $147.82 \pm 12.82$& $220.61 \pm 13.56$& $170.30 \pm 10.58$& $216.47 \pm 13.36$& $199.22 \pm 13.34$ \\
RMS & $100.00 \pm 5.31$& $100.00 \pm 6.81$& $100.00 \pm 6.79$& $100.00 \pm 8.33$& $100.00 \pm 12.27$ \\
RMS-MR & $67.23 \pm 5.32$& $51.63 \pm 4.53$& $56.07 \pm 3.40$& $56.33 \pm 7.38$& $54.28 \pm 6.73$ \\
RMS-SL & $107.91 \pm 7.99$& $103.45 \pm 10.36$& $90.61 \pm 6.25$& $114.05 \pm 18.99$& $106.35 \pm 10.45$ \\
SGFS & $142.34 \pm 5.55$& $153.14 \pm 8.43$& $127.02 \pm 11.76$& $193.66 \pm 10.14$& $150.93 \pm 8.58$ \\
SGFS-MR & $188.74 \pm 48.01$& $178.01 \pm 22.31$& $119.30 \pm 16.79$& $256.76 \pm 79.99$& $196.23 \pm 31.54$ \\
SGFS-SL & $88.45 \pm 19.15$& $71.34 \pm 8.41$& $60.82 \pm 11.43$& $99.20 \pm 24.01$& $81.54 \pm 13.08$ \\
ConstSGD & $110.95 \pm 7.49$& $109.21 \pm 7.49$& $107.34 \pm 7.72$& $116.68 \pm 12.45$& $111.59 \pm 9.00$ \\
ConstSGD-MR & $38.16 \pm 12.76$& $13.18 \pm 1.90$& $24.87 \pm 5.29$& $15.80 \pm 4.68$& $14.76 \pm 1.94$ \\
ConstSGD-SL & $73.90 \pm 16.27$& $51.23 \pm 5.90$& $52.37 \pm 9.78$& $65.17 \pm 32.75$& $56.33 \pm 9.32$ \\
EpsGreedyRMS & $99.92 \pm 4.05$& $100.64 \pm 6.12$& $100.74 \pm 7.09$& $89.64 \pm 5.27$& $97.95 \pm 12.20$ \\
EpsGreedyRMS-SL & $242.38 \pm 13.74$& $267.58 \pm 25.50$& $306.46 \pm 9.59$& $131.72 \pm 14.07$& $205.68 \pm 20.47$ \\
EpsGreedyRMS-MR & $60.25 \pm 8.41$& $52.85 \pm 5.24$& $51.73 \pm 5.03$& $53.57 \pm 10.19$& $49.82 \pm 5.50$ \\
LinDiagPost & $81.33 \pm 3.25$& $21.36 \pm 1.67$& $42.80 \pm 2.73$& $11.94 \pm 0.92$& $22.46 \pm 2.64$ \\
LinDiagPost-MR & $84.63 \pm 15.24$& $24.04 \pm 4.11$& $45.32 \pm 3.17$& $12.38 \pm 2.29$& $19.43 \pm 1.25$ \\
LinDiagPost-SL & $85.61 \pm 10.53$& $27.27 \pm 3.25$& $55.19 \pm 5.90$& $11.31 \pm 1.00$& $21.42 \pm 2.62$ \\
LinDiagPrecPost & $85.47 \pm 9.51$& $25.24 \pm 1.97$& $59.29 \pm 5.03$& $12.97 \pm 1.35$& $22.99 \pm 2.70$ \\
LinDiagPrecPost-MR & $93.74 \pm 19.87$& $24.97 \pm 2.05$& $54.88 \pm 4.57$& $11.88 \pm 1.42$& $20.25 \pm 1.62$ \\
LinDiagPrecPost-SL & $86.35 \pm 8.15$& $25.95 \pm 3.96$& $55.29 \pm 4.83$& $12.16 \pm 1.80$& $21.61 \pm 2.34$ \\
LinGreedy & $78.87 \pm 11.13$& $21.43 \pm 1.42$& $56.02 \pm 3.93$& $3.52 \pm 0.46$& $13.96 \pm 1.61$ \\
LinGreedy ($\epsilon =0.01$) & $73.55 \pm 3.39$& $21.32 \pm 1.77$& $55.23 \pm 4.59$& $3.64 \pm 0.42$& $13.74 \pm 1.84$ \\
LinGreedy ($\epsilon =0.05$) & $73.92 \pm 2.98$& $20.00 \pm 1.64$& $52.66 \pm 3.54$& $3.51 \pm 0.33$& $13.09 \pm 1.76$ \\
LinPost & $93.53 \pm 3.58$& $25.93 \pm 2.65$& $64.87 \pm 5.03$& $23.19 \pm 1.53$& $38.20 \pm 3.64$ \\
LinPost-MR & $96.52 \pm 12.06$& $33.95 \pm 6.89$& $58.76 \pm 4.66$& $26.40 \pm 3.62$& $33.74 \pm 1.37$ \\
LinPost-SL & $98.21 \pm 8.85$& $27.45 \pm 3.39$& $61.25 \pm 6.07$& $22.55 \pm 2.42$& $36.00 \pm 2.94$ \\
LinFullDiagPost & $80.47 \pm 3.28$& $25.46 \pm 2.57$& $48.37 \pm 3.15$& $15.35 \pm 1.42$& $24.18 \pm 2.58$ \\
LinFullDiagPost-MR & $81.25 \pm 6.02$& $27.68 \pm 2.58$& $57.34 \pm 6.74$& $14.34 \pm 2.52$& $20.90 \pm 1.90$ \\
LinFullDiagPost-SL & $77.71 \pm 3.45$& $25.78 \pm 2.46$& $54.59 \pm 5.23$& $14.39 \pm 1.51$& $23.10 \pm 3.86$ \\
LinFullDiagPrecPost & $80.75 \pm 3.03$& $26.72 \pm 2.01$& $58.37 \pm 4.05$& $15.18 \pm 1.46$& $22.56 \pm 2.16$ \\
LinFullDiagPrecPost-MR & $84.67 \pm 9.11$& $27.35 \pm 2.81$& $56.35 \pm 6.31$& $14.58 \pm 2.03$& $22.05 \pm 1.70$ \\
LinFullDiagPrecPost-SL & $77.85 \pm 4.66$& $25.13 \pm 2.30$& $53.79 \pm 4.76$& $13.68 \pm 0.90$& $22.69 \pm 2.44$ \\
LinFullPost & $94.41 \pm 3.70$& $27.22 \pm 1.88$& $65.02 \pm 4.04$& $26.00 \pm 2.05$& $40.23 \pm 3.46$ \\
LinFullPost-MR & $99.09 \pm 5.90$& $28.90 \pm 2.67$& $62.19 \pm 4.79$& $29.87 \pm 3.17$& $38.99 \pm 3.01$ \\
LinFullPost-SL & $99.33 \pm 5.56$& $29.80 \pm 2.58$& $63.71 \pm 5.07$& $28.95 \pm 3.94$& $38.72 \pm 2.50$ \\
ParamNoise & $145.32 \pm 7.94$& $170.52 \pm 13.40$& $129.23 \pm 12.58$& $228.62 \pm 20.71$& $185.53 \pm 22.58$ \\
ParamNoise-MR & $62.50 \pm 13.75$& $42.40 \pm 6.77$& $41.12 \pm 8.23$& $60.75 \pm 9.18$& $50.05 \pm 6.11$ \\
ParamNoise-SL & $33.49 \pm 2.28$& $13.23 \pm 1.56$& $22.01 \pm 1.51$& $16.13 \pm 3.81$& $16.29 \pm 2.59$ \\
Uniform & \bm{$0.16 \pm 0.01$}& \bm{$0.21 \pm 0.02$}& \bm{$0.22 \pm 0.01$}& \bm{$0.18 \pm 0.03$}& \bm{$0.19 \pm 0.02$} \\
\bottomrule
\end{tabular}

